CLGNN: A Contrastive Learning-based GNN Model for Betweenness Centrality Prediction on Temporal Graphs

Temporal Betweenness Centrality (TBC) measures how often a node appears on optimal temporal paths, reflecting its importance in temporal networks. However, exact computation is highly expensive, and real-world TBC distributions are extremely imbalanced. The severe imbalance leads learning-based models to overfit to zero-centrality nodes, resulting in inaccurate TBC predictions and failure to identify truly central nodes. Existing graph neural network (GNN) methods either fail to handle such imbalance or ignore temporal dependencies altogether. To address these issues, we propose a scalable and inductive contrastive learning-based GNN (CLGNN) for accurate and efficient TBC prediction. CLGNN builds an instance graph to preserve path validity and temporal order, then encodes structural and temporal features using dual aggregation, i.e., mean and edge-to-node multi-head attention mechanisms, enhanced by temporal path count and time encodings. A stability-based clustering-guided contrastive module (KContrastNet) is introduced to separate high-, median-, and low-centrality nodes in representation space, mitigating class imbalance, while a regression module (ValueNet) estimates TBC values. CLGNN also supports multiple optimal path definitions to accommodate diverse temporal semantics. Extensive experiments demonstrate the effectiveness and efficiency of CLGNN across diverse benchmarks. CLGNN achieves up to a 663.7~$\times$ speedup compared to state-of-the-art exact TBC computation methods. It outperforms leading static GNN baselines with up to 31.4~$\times$ lower MAE and 16.7~$\times$ higher Spearman correlation, and surpasses state-of-the-art temporal GNNs with up to 5.7~$\times$ lower MAE and 3.9~$\times$ higher Spearman correlation.

==> copy.tex <==
\section{Proposed model}
\label{sec:proposedmodel}

% 插入整体框架图+概述性的每一个块
\begin{figure*}[htbp]  % 控制图片位置
\vspace{-16pt}
  \centering  % 图片居中
  \includegraphics[width=\textwidth]{CLGNN.pdf}  % 图片路径和文件名
  \caption{Overview of the Proposed Model: CLGNN}  % 图片说明文字
  \label{fig:CLGNNarchitecture}  % 图片的标签，用于引用
\vspace{-10pt}
\end{figure*}
To effectively predict TBC under strong data imbalance, we propose a contrastive learning-based GNN model, CLGNN, as illustrated in Figure~\ref{fig:CLGNNarchitecture}. CLGNN is composed of two main components, i.e., a representation module and a prediction module. We describe each module in detail below. 


\subsection{Representation Module}\label{sec:rep}
%\textbf{Instance graph construction and temporal path counting procedure.}
To capture the temporal paths and preserve the temporal dependencies, we first transform temporal graphs into an instance-level structure, where each node $v$ is associated with the set $T_{out}(v)$ of the timestamps attached with $v$'s outgoing edges. In addition, for each node $u$ and its outgoing edge $(u,v,t)$, we maintain the number of valid temporal paths, denoted as:
\[
P(u,v,t) = \sum_{t_v \in T_{\mathrm{out}}(v)} \mathbb{I}(t_v-t),
\]
where $\mathbb{I}(x)$ is an indicator function that defined as: $\mathbb{I}(x) = 
\begin{cases}
1, & \text{if } x > 0 \\
0, & \text{otherwise}
\end{cases}$. If $P(u,v,t)=0$, then the message generated by node $u$ will not be transmitted to node $v$ through the edge with timestamp $t$ during the message passing process.

\textbf{Path-Time dual-aware mechanism.}

It combines continuous time encoding and temporal path count encoding, jointly capturing temporal dependencies and relevant path information in the message passing process.

\textbf{\textbullet~Continuous Time Encoding.} We employed the approach in \cite{xu2020inductive}, which applies Bochner's theorem and Monte Carlo integral to map a temporal domain \( T = [0, t_{\text{max}}] \) to the \( d \)-dimensional vector space. 
\[
\Phi_{time}(t) = \sqrt{\frac{1}{d_T}} \left[ \cos(\omega_1 t), \sin(\omega_1 t), \dots, \cos(\omega_{d_T} t), \sin(\omega_{d_T} t) \right]^T ,
\]
where \( d_T \) is the finite dimension and \( \omega = (\omega_1, \dots, \omega_{d_T})^T \) are learnable parameters.

\textbf{\textbullet~Temporal Path Count Encoding.}
Temporal path count encoding processes the number of temporal paths to provide stable and efficient input features for the neural network. It is defined as: 
\[
P(u, v, t) \xrightarrow{\text{log-transformed value}} \log(1 + P(u, v, t)),
\]
\[
\Phi_{path}(u,v,t) = \text{MLP}(\text{reshape}( \log(1 + P(u,v,t)) )),
\]
where the reshaping operation \( \text{reshape}(1, 1) \) converts the scalar into a suitable format for input into the network. Note that the path count \( P(u, v, t) \) undergoes a \( \log(1 + P) \) transformation, which aims to compress the influence of large path values on model training, alleviating gradient explosion issues while preserving non-negativity and the distinguishability of the values.

\textbf{Message Function.}

For each interaction event $e=(u,v,t)$, a message is computed to update the representation of node $v$. Specifically, the message at layer $l$ is defined as:
\[
m^l_{uv}(t) = \left h^{l-1}_{u}(t^-) || h^{l-1}_{v}(t^-)||\Phi_{time}(t-t^-) || \Phi_{path}(u,v,t) \right,
\]
where $h^{l-1}_{u}(t^-)$, $h^{l-1}_{v}(t^-) \in \mathbb{R}^{d}$ are the hidden representation for node \( u \) and \( v \) in the previous layer (the $l-1$ layer) of the neural network just before time \( t \) (i.e., from the time of the previous interaction involving \( u \) and \( v \)), and $||$ denotes concatenation. %and  $\text{msg}(\cdot)$ is the message function, implemented as a concatenation of all inputs. 
The computed message $m^l_{uv}(t)$ is then passed into the aggregation function and contributes to the update of node $v$'s embedding at layer $l$.

\textbf{Dual Message Aggregator Mechanism.}
Since each node typically interacts with multiple neighbors and may receive multiple messages from the same neighbor at different times, there exist two levels of message aggregation: across edges and across nodes. To address this, we employ a dual aggregation mechanism, i.e., mean aggregation and edge-to-node multi-head attention, to balance the model’s stability and flexibility.


\textbf{\textbullet~Mean aggregation (node-level).} 
Mean aggregation performs aggregation at the node level, ensuring that all neighbors contribute equally to the target node’s representation. 

At the $l$-th layer, the mean-aggregated message received by node \( v \) at time \( t \) is computed as:
\[
\bar{h}^l_v(t) = \frac{1}{|N_{\text{in}}(v)|} \sum_{u \in N_{\text{in}}(v)} \left( \sum_{t_x \in T_{uv}}  \frac{P(u, v, t_x)}{\sum_{t_x' \in {T}_{uv}} P(u, v, t_x')}  \cdot m^l_{uv}(t_x) \right),
\]
where $N_{in}(v)$ is the set of $v$'s in-neighbors; $T_{uv}$ is the set of timestamps associated with all edges from $u$ to $v$; \( m^l_{uv}(t_x) \) is the message computed at time \( t_x \) in the $l$-th layer. %This formulation ensures a normalized, path-aware aggregation across temporal edges and neighbors. 
Notably, only temporal paths that are reachable (i.e., those with \( P(u, v, t_x) > 0 \)) are considered in the aggregation. 

\textbf{\textbullet~Edge-to-node multi-head attention (edge-level).}
This mechanism computes attention for each edge connected to a node, ensuring that all temporal edges contribute to the node's representation update.  
The input matrix of the $l$-th attention layer is:
\[
M_v^l(t) = \left[ m^l_{uv}(t_x) \right]_{\forall(u,v, t_x) \in E_{in}(v),P(u, v, t_x) > 0 }^T, 
%\quad \text{s.t.} \quad u \in N_{\text{in}}(v),\; t_i \in T_{uv},\; P(u, v, t_i) > 0
\]
$E_{in}(v)$ is the set of $v$'s incoming edges. %The resulting matrix \( M^l(t) \in \mathbb{R}^{L \times d} \), where $L$ denote the number of time-respecting messages received  from node $v's$ incoming edges, i.e., the number of messages with $P(u, v, t_x) > 0$. 
Then \( M^l(t) \) is projected into query, key, and value spaces: $Q^l(t) = [h^{l-1}_{v}(t^-) \,||\, h^{l-1}_{v}(t^-) \,||\, \Phi_{\text{time}}(t - t^-) \,||\, \Phi_{\text{path}}(u, v, t)] \cdot W_Q$; $K^l(t) = M^l(t) \cdot W_K$; $V^l(t) = M^l(t) \cdot W_V$, where \( W_Q, W_K, W_V \in \mathbb{R}^{(d + d_T) \times d_h} \) are learnable projection matrices, and \( d_h \) is the hidden dimension. 

Next, the scaled dot-product attention is used in attention layers.  The aggregated message for node $v$ at the $l$-th layer, computed via the multi-head attention mechanism, is given by:
\[
\tilde{h}_{v}^l(t)=\text{Attn}(Q^l(t), K^l(t), V^l(t)) = \text{softmax} \left( \frac{Q^l(t)(K^l(t))^T}{\sqrt{d_h}} \right) V^l(t) \in \mathbb{R}^{d_h}
\]
\textbf{Embedding.}
The final embedding of node \( v \) at time \( t \), denoted as \( h^l_v(t) \),  is obtained by combining the outputs of mean aggregation and edge-to-node multi-head attention:
\begin{align*}
h^l_v(t) &= \lambda \cdot h_v^{l(\text{mean})}(t) + (1 - \lambda) \cdot h_v^{l(\text{attention})}(t), \\
h_v^{l(\text{mean})}(t) &= \text{MLP}( \bar{h}_v^{l}(t) \parallel h_v^{l-1}(t)), \\
h_v^{l(\text{attention})}(t) &= \text{MLP}\left( \tilde{h}_v^{l(0)}(t) \parallel \tilde{h}_v^{l(1)}(t) \parallel \cdots \parallel \tilde{h}_v^{l(k-1)}(t) \parallel h_v^{l-1}(t) \right),
\end{align*}
where \( k \) is the number of heads, and \( h_v^{l(j)}(t) \) \((0 \leq j < k)\) is the dot-product attention output of the \( j \)-th head.   \( \lambda \) is a coefficient that balances the contribution of the two aggregation types. This weighted combination allows the model to trade off between the stability of equal neighbor contributions and the flexibility of dynamic attention-based relevance, enabling expressive temporal node representations.



 \subsection{Prediction Module}\label{sec:pre}
To address the imbalance in temporal betweenness centrality values and enhance the model's sensitivity to rare but important nodes, we design two complementary components, i.e., KContrastNet and ValueNet, in the prediction module.

\textbf{KContrastNet.}
 KContrastNet employs a contrastive learning strategy to effectively distinguish features among low-, medium-, and high-value nodes in TBC prediction. To enhance the selection of positive and negative sample pairs, we first introduce a stability-based clustering approach that identifies the optimal number \(k\) of clusters in the node representation space. 

\textbf{\textbullet~Stability-based clustering method.}

Traditional methods for choosing the number of clusters, such as the elbow method~\cite{thorndike1953belongs} or silhouette score~\cite{rousseeuw1987silhouettes}, often struggle with noisy data or class imbalance, leading to unstable results. To address this, we propose a stability-based clustering method that combines bootstrap resampling~\cite{2012Selection} with K-means clustering~\cite{hartigan1979algorithm} to estimate the optimal number of clusters. To improve efficiency, we first perform stratified random sampling on the original dataset \( F \) to obtain a reduced subset \( F^n \)  (e.g., 40\% of the original size) that retains the original distribution.  Bootstrap resampling is then applied on \( F^n \) to generate \( B \)  independent sample pairs \( \{(X_i, Y_i)\}_{i=1}^B \), ensuring each drawn independently and identically from the empirical distribution (a formal justification is provided in Appendix~\ref{appendix:iid}). For each pair and each candidate cluster number \( k \in \{2, \dots, K\} \), we run k-means separately on  \( X_i \) and \( Y_i \) to obtain two cluster assignments \( \psi_{X_i}\) and \( \psi_{Y_i}\), respectively. We then compute the clustering distance between these assignments and average the results over all \( B \) pairs to obtain a clustering instability, as formally defined below.

%附录放证明过程
%可放附录
\begin{definition}\label{defn:CD}
{\bf (Clustering Distance)}. The clustering distance between two clustering results $\psi_{X_i}$ and $\psi_{Y_i}$ is defined as:
\[
d(\psi_{X_i}, \psi_{Y_i}) = E_{x, y \in (X_i \cap Y_i)} \left[ \delta(\psi_{X_i}(x), \psi_{X_i}(y)) - \delta(\psi_{Y_i}(x), \psi_{Y_i}(y)) \right],
\]
where \( E \) denotes the expectation operator, computed over all possible samples \( x \) and \( y \). $\psi_{X_i}(x)$ denotes the cluster label assigned to sample $x$ in the clustering result $\psi_{X_i}$. The function $\delta(a, b)$ is the Kronecker Delta, defined as: $
\delta(a, b) = 
\begin{cases}
1, & \text{if } a = b, \\
0, & \text{if } a \neq b.
\end{cases}.
$
\end{definition}
%可放附录
\begin{definition}\label{defn:CI}
{\bf (K-means Clustering Instability)}. 
The clustering instability quantifies the variation in clustering results across different resamples and is defined as:
\[
\hat{s}_B(\psi, k, n) = \frac{1}{B} \sum_{i=1}^{B} d\left(\text{KMeans}(X_{i}, k), \text{KMeans}(Y_{i}, k)\right),
\]
$\psi$ is the clustering results of \text{KMeans} function and 
$d(\cdot,\cdot)$ is the clustering distance defined above.
% where $X_i$ and $Y_i$ are two independent random samples drawn from the data distribution $F_n$, and $d_F$ is the clustering distance. 
\end{definition}
Finally, the optimal number of clusters  $\hat{k}$ $=$ $\arg~\min_{2\leq k \leq K}$ $\hat{s}_B$ $(\psi,$ $k,$ $n)$ by minimizing the instability. Statistical properties of the estimator, including unbiasedness and consistency, are detailed in Appendix~\ref{appendix:instability_consistency}. And the complete algorithm and its complexity analysis are provided in Appendix~\ref{appendix:algorithm}.

\textbf{\textbullet~Contrastive Learning.}
% As shown in Fig.~\ref{fig:pre_architecture}, 
After clustering, each node is assigned a cluster label, which guides the construction of supervised contrastive learning pairs.   To ensure that positive samples are both semantically meaningful and structurally consistent, we introduce a conditional sampling strategy. Specifically, positive samples are formed by selecting nodes from the same cluster that have similar TBC values, while negative samples are chosen from the same cluster but with large TBC differences. A theoretical justification for choosing within-cluster sampling alternatives is provided in Appendix~\ref{appendix:intracluster}.


Positive sample selection: let \( \mathcal{S^+}(u) \) be the set of positive samples for node \( u \), defined as:
\[
\mathcal{S}^+(u) = \left\{ v \mid \delta(\psi(u), \psi(v))=1, 0<\left| TBC(u) - TBC(v) \right| \leq \gamma_{pos} \cdot TBC_{median} \right\},
\]
where \( \gamma_{pos} \in (0,1) \) is a similarity threshold  (e.g., 0.5). The use of the median TBC value ensures robustness against outliers and skewed distributions, improving the stability of contrastive thresholds. 

Negative sample selection: let \( \mathcal{S}^-(u) \) be the set of negative samples for node \( u \), defined as:
\[
\mathcal{S}^-(u) = \left\{ v \mid \delta(\psi(u), \psi(v))=1, \left| TBC(u) - TBC(v) \right| \geq \gamma_{neg} \cdot TBC_{median} \right\},
\]
where \( \gamma_{neg} \) (e.g., 0.5) is a dissimilarity threshold.

The contrastive re-weighted loss \( \mathcal{L}_{\text{contrast}} \) is then computed across all clusters, encouraging the embeddings of positive pairs to be closer while pushing negative pairs apart, weighted by their semantic similarity. The loss is defined as follows:

\[
\mathcal{L}_{\text{contrast}} = \sum_{i=1}^{\hat{k}} \sum_{u \in \psi_i} -\log \frac{\sum\limits_{v \in \mathcal{S}^+(u)} \exp\left( \beta_{uv} \cdot \text{sim}(\mathbf{h}_u, \mathbf{h}_v)/\tau \right)}{\sum\limits_{v \in \mathcal{S}^+(u)} \exp\left( \beta_{uv} \cdot \text{sim}(\mathbf{h}_u, \mathbf{h}_v)/\tau \right) + \sum\limits_{w \in \mathcal{S}^-(u)} \exp\left( \beta_{uw} \cdot\text{sim}(\mathbf{h}_u, \mathbf{h}_w)/\tau \right)}
\]
where \(\mathbf{h}_u\) is the node embedding of GNN introduced in section~\ref{sec:rep},  \( \text{sim}(\cdot, \cdot) \) denote the  dot product similarity.  \( \tau \) is the temperature parameter of InfoNCE~\cite{InfoNCE}.  the pairwise weights for positive samples \( \beta_{uv} \) and negative samples \( \beta_{uw} \) are calculated as:
\[
\beta_{uv} = \frac{TBC_{median}\cdot \gamma_{pos}}{\left| TBC(u) - TBC(v) \right|} , ~~~~
\beta_{uw} = \frac{\left| TBC(u) - TBC(w) \right|}{TBC_{median}\cdot \gamma_{neg} } 
\]
The weight design ensures that node embeddings are adjusted in proportion to their TBC differences. For positive samples,  the smaller the TBC gap between nodes $u$ and $v$, the larger the weight \( \beta_{uv} \),  encouraging the model to learn more from highly similar pairs. For negative samples, the weight   \( \beta_{uw} \) increases with larger TBC differences, emphasizing separation from more dissimilar nodes. A theoretical analysis of this contrastive loss design is provided in Appendix~\ref{appendix:contrastive_theory}. 


\textbf{ValueNet.}
%In ValueNet, we predict the TBC values of nodes based on the representations learned in the representation module described in Section~\ref{sec:rep}. 
For each node \( v \in V \), the TBC score at the largest timestamp (i.e., lateset time) \( t_{\max} \), denoted as \( \text{TBC}_{t_{max}}(v) \),  represents the final TBC value of \( v \) under the full-graph setting. It is predicted using a three-layer MLP with ReLU activations:
\[
TBC(v) = TBC_{t_{\max}}(v) = \text{MLP}(h_v^l(t_{\max})),
\]
where \( h_v^l(t_{max}) \) is the output representation of node \( v \) from the last GNN layer at time \( t_{max} \).

\textbf{Total Loss Function.}
%To jointly optimize the TBC regression task and the contrastive representation learning, we design 
A weighted total loss function that balances the regression loss and the contrastive loss is defined as:
\[
\mathcal{L}_{\text{total}} = \alpha \cdot \mathcal{L}_{\text{contrast}} + (1 - \alpha) \cdot \mathcal{L}_{\text{regress}}
\]
\textcolor{red}{where \( \mathcal{L}_{\text{regress}} \) is the regression loss (e.g., MAE), and \( \mathcal{L}_{\text{contrast}} \) is the contrastive re-weighted loss as described above. The hyperparameter \( \alpha \in [0,1] \) controls the trade-off between the two objectives.

